Hyper Evidential Deep Learning to Quantify Composite Classification Uncertainty

Deep neural networks (DNNs) have been shown to perform well on exclusive, multi-class classification tasks. However, when different classes have similar visual features, it becomes challenging for human annotators to differentiate them. This scenario necessitates the use of composite class labels. In this paper, we propose a novel framework called Hyper-Evidential Neural Network (HENN) that explicitly models predictive uncertainty due to composite class labels in training data in the context of the belief theory called Subjective Logic (SL). By placing a grouped Dirichlet distribution on the class probabilities, we treat predictions of a neural network as parameters of hyper-subjective opinions and learn the network that collects both single and composite evidence leading to these hyper-opinions by a deterministic DNN from data. We introduce a new uncertainty type called vagueness originally designed for hyper-opinions in SL to quantify composite classification uncertainty for DNNs. Our results demonstrate that HENN outperforms its state-of-the-art counterparts based on four image datasets. The code and datasets are available at: https://github.com/Hugo101/HyperEvidentialNN.

==> limitation.tex <==
\vspace{-2mm}
The potential applications for the proposed HENN and \textit{vagueness} uncertainty are vast, ranging from medical diagnosis systems to autonomous driving. However, it's important to note that GDD can only map hyper-opinions with disjointing composite labels and is unable to handle overlapping composite label scenarios. While the Hyper-Dirichlet distribution (HDD)~\citep{JSSv033i11} could be used as an alternative, UACE loss based on HDD does not have an analytical form due to HDD's normalizing constant without analytical form. It is possible to use Monte Carlo (MC) techniques to approximate the UACE function. However, as each training example has a different Hyper-Dirichlet distribution and hence a different UACE loss, we need to apply MC to the UACE loss of each training example separately, which is not scalable to a large training dataset. Therefore, this remains an area for future research.
\vspace{-2ex}
